MaskEval: Weighted MLM-Based Evaluation for Text Summarization and Simplification

In text summarization and simplification, system outputs must be evaluated along multiple dimensions such as relevance, factual consistency, fluency, and grammaticality, and a wide range of possible outputs could be of high quality. These properties make the development of an adaptable, reference-less evaluation metric both necessary and challenging. We introduce MaskEval, a reference-less metric for text summarization and simplification that operates by performing masked language modeling (MLM) on the concatenation of the candidate and the source texts. It features an attention-like weighting mechanism to modulate the relative importance of each MLM step, which crucially allows it to be adapted to evaluate different quality dimensions. We demonstrate its effectiveness on English summarization and simplification in terms of correlations with human judgments, and explore transfer scenarios between the two tasks.

==> tab/english-summarisation-results.tex <==
\begin{table*}[!!ht]
\centering\small
\iffalse
\begin{tabular}{lcccccc}
\toprule
\multicolumn{7}{c}{\bf{SummEval}} \\
\midrule
                    & \#Ref & Consistency & Coherence & Fluency & Relevance & Ave. \\
\midrule
Perplexity & 0   &  -3.1 & 15.7 & 8.9 & 19.8 & 10.3
\\
Length & 0    & 8.1 & 8.6 & -2.9 & 26.6 & 10.1
  \\
\midrule
ROUGE-1             & 11    & 18.1        & 20.1      & 14.9    & 35.6      & 22.2    \\
ROUGE-L             & 11    & 15.7        & 15.6      & 13.8    & 33.4      & 19.6    \\
BLEU                & 11    & 17.5        & 22.0      & 13.7    & 35.6      & 22.2    \\
BERTScore-f         & 11    & 20.3        & 18.5      & 21.6    & 31.9      & 23.1    \\ \midrule
ROUGE-1             & 1     & 11.0        & 9.8       & 7.5     & 18.9      & 11.8    \\
ROUGE-L             & 1     & 8.2         & 7.3       & 5.7     & 13.5      & 8.7     \\
BLEU                & 1     & 8.9         & 3.9       & 4.0     & 12.7      & 7.4     \\
BERTScore-f         & 1     & 8.7         & 9.8       & 10.6    & 17.9      & 11.8    \\ \midrule
% Spearman: BARTScore         & 1     & 37.8        & \textbf{40.7}     & 33.8    & 36.8    & \textbf{37.3}   \\ 
BARTScore         & 0     & 37.1        & \textbf{41.3}    & 33.1    & \textbf{44.8}    & \textbf{39.1} \\ 
% Spearman: PRISM               & 0    & 34.5         & 24.9       & 25.4     & 21.2      & 26.5     \\
PRISM               & 0    & 29.7         & 28.1       & 24.8     & 29.7     & 28.1     \\
SummaQA             & 0     & 8.3         & 8.0       & -2.9    & 26.2      & 9.9     \\
QAGS                & 0     & 20.4        & 7.7       & 16.8    & 9.1       & 13.7    \\
%QuestEval$_{W = uniform}$  & 0     & 43.7        & 22.9      & 28.2    & 37.5      & 33.1    \\
QuestEval & 0     & 42.0       & 24.0      & 28.4    & 39.2      & 33.5    \\ \midrule

\modelnamenoxs$_{\text{Summ}\; W=\text{uniform}}$  & 0 & \textbf{44.6}       & 27.6      & \textbf{40.6}   & 35.6     & 37.1    \\
\modelnamenoxs$_{\text{Simpl}\; W=\text{uniform}}$  & 0 &  44.6 & 29.4 & 37.6 & 35.2 & 36.7 \\
\ \ \ \qquad\qquad\qquad$_{W=\text{opt\_\texttt{Flu}}}$ & 0 & 41.7 &  24.8 & 34.7 & 31.0 & 33.1  \\
\ \ \ \qquad\qquad\qquad$_{W=\text{opt\_\texttt{Sim}}}$ & 0 & 40.8 & 24.8 & 34.2 & 30.0 & 32.5  \\
\ \ \ \qquad\qquad\qquad$_{W=\text{opt\_\texttt{Mea}}}$ & 0 & 42.4 & 25.1 & 35.3 & 31.0 & 33.5 \\
%\hspace{15mm}$_{\textrm{Mask\_SRC}}$  & 0     & 17.1        & 17.7  & 16.1      & 28.9    & 20.0\\
%\hspace{15mm}$_{\textrm{MASK\_HYP}}$   & 0     & \textbf{50.0}        & 26.4      & \textbf{46.3}   & 29.2      & \textbf{38.0} \\
\bottomrule
\end{tabular}
\fi

\begin{tabular}{c@{}c@{}c}
%\begin{tabular}{l@{~~}r@{~~~}r@{~~~}r@{~~~}r@{~~~}r}
\setlength{\tabcolsep}{4pt}
\begin{tabular}{lrrrrr} % Default value: 6pt
\toprule
\multicolumn{6}{c}{\bf{SummEval, reference-less}} \\
\midrule
                    & Cons. & Coh. & Flu. & Rel. & Ave. \\
\midrule
Perplexity &  -3.1 & 15.7 & 8.9 & 19.8 & 10.3
\\
Length  & 8.1 & 8.6 & -2.9 & 26.6 & 10.1
  \\
\midrule
BARTScore           & 37.1        & \textbf{41.3}    & 33.1    & \textbf{44.8}    & \textbf{39.1} \\ 
PRISM                 & 29.7         & 28.1       & 24.8     & 29.7     & 28.1     \\
SummaQA               & 8.3         & 8.0       & -2.9    & 26.2      & 9.9     \\
QAGS                   & 20.4        & 7.7       & 16.8    & 9.1       & 13.7    \\
QuestEval &    42.0       & 24.0      & 28.4    & 39.2      & 33.5    \\ \midrule

\modelnamenoxs$_{\text{Summ}\ \text{uniform}}$  & \textbf{44.6}       & 27.6      & \textbf{40.6}   & 35.6     & 37.1    \\
\modelnamenoxs$_{\text{Simpl}\ \text{uniform}}$  &  44.6 & 29.4 & 37.6 & 35.2 & 36.7 \\
\ \ \ \qquad\qquad\qquad$_{\text{opt\_\texttt{Flu}}}$ & 41.7 &  24.8 & 34.7 & 31.0 & 33.1  \\
\ \ \ \qquad\qquad\qquad$_{\text{opt\_\texttt{Sim}}}$ & 40.8 & 24.8 & 34.2 & 30.0 & 32.5  \\
\ \ \ \qquad\qquad\qquad$_{\text{opt\_\texttt{Mea}}}$ & 42.4 & 25.1 & 35.3 & 31.0 & 33.5 \\
\bottomrule
\end{tabular}
&~~~~~~&
%\begin{tabular}{l@{~~}r@{~~~}r@{~~~}r@{~~~}r@{~~~}r@{~~~}r}
\setlength{\tabcolsep}{4pt}
\begin{tabular}{lrrrrrr} % Default value: 6pt
\toprule
\multicolumn{7}{c}{\bf{SummEval, with reference(s)}} \\
\midrule
                    & \#Ref & Cons. & Coh. & Flu. & Rel. & Ave. \\
\midrule
ROUGE-1             & 11    & 18.1        & 20.1      & 14.9    & 35.6      & 22.2    \\
ROUGE-L             & 11    & 15.7        & 15.6      & 13.8    & 33.4      & 19.6    \\
BLEU                & 11    & 17.5        & 22.0      & 13.7    & 35.6      & 22.2    \\
BERTScore-f         & 11    & 20.3        & 18.5      & 21.6    & 31.9      & 23.1    \\ \midrule
ROUGE-1             & 1     & 11.0        & 9.8       & 7.5     & 18.9      & 11.8    \\
ROUGE-L             & 1     & 8.2         & 7.3       & 5.7     & 13.5      & 8.7     \\
BLEU                & 1     & 8.9         & 3.9       & 4.0     & 12.7      & 7.4     \\
BERTScore-f         & 1     & 8.7         & 9.8       & 10.6    & 17.9      & 11.8    \\ 
\bottomrule
\end{tabular}
\end{tabular}





\begin{tabular}{lrrrrr}
\toprule
\multicolumn{6}{c}{\bf{SummEval subset (attention weight module's test set), reference-less}} \\
\midrule
                & Consistency & Coherence & Fluency & Relevance & Average \\
\midrule
\modelnamenoxs$_{\text{Summ}\ \text{uniform}}$ & 44.1     & 27.3      & 42.3   & 35.5     & 37.3 \\
\modelnamenoxs$_{\text{Summ}\ \text{learned}}$ &   46.0  & 29.3 & 44.9 & 40.1 & 40.1\\
\bottomrule
\end{tabular}
    \caption{English summarization results on the SummEval dataset (Pearson correlation). The tables on top report results on the entire dataset (1600 summary-source pairs). Baseline non-QA metrics results are as reported in \citep{DBLP:journals/corr/abs-2007-12626}; QA-based metrics results are as reported in \citep{QuestEval}. %\modelname results are computed by uniformly weighting each text segment. 
    The bottom section reports results on the subset (900 pairs).} %On $\text{learned}$ each entry corresponds to \modelname using a weighting function that learned to optimize for the corresponding dimension.}
    \label{tab:english_summarization}
\end{table*}

==> tab/simplification-results.tex <==
\begin{table*}[!ht]
\centering\small
\begin{tabular}{lccccccc}
\toprule
\multicolumn{8}{c}{\bf{Simplification}} \\
\midrule
{} & \bf{\#Ref} & \multicolumn{3}{c}{\bf{System-generated simplifications}} & \multicolumn{3}{c}{\bf{Human-written simplifications}}\\
& {} & Fluency & Simplicity & Meaning & Fluency & Simplicity & Meaning \\
\midrule
Perplexity & 0 & 22.9$^{*}$ &	20.4$^{*}$&	23.1$^{*}$&	11.0&	-4.8&	27.1
  \\
Length & 0 & 2.5 &	-0.8 &	19.4 &	-31.3 &	-42.8 &	6.4
 \\
\midrule
ROUGE-1 & 10 & 42.0$^{**}$ &	42.4$^{**}$ &	61.8$^{**}$ &	10 &	-8.3 &	35.2
 \\
ROUGE-L & 10 & 40.9$^{**}$ &	41.0$^{**}$ &	59.4$^{**}$ &	15.5 &	-4.7 &	28.6
 \\
BLEU & 10 & 28.9$^{**}$ &	29.5$^{**}$ &	47.6$^{**}$ &	47.6 &	34.0 &	22.7
\\
BERTScore-f & 10 & \textbf{58.0}$^{**}$ &	\textbf{54.7}$^{**}$ 	 & \textbf{73.4}$^{**}$	 &51.3	 &36.3	 &23.8
  \\
\midrule
ROUGE-1 & 1 & 33.7$^{**}$ &	31.2$^{**}$ & 47.9$^{**}$ &	3.6 &	-7.2 &	9.0
\\
ROUGE-L & 1 & 31.8$^{**}$ &	28.5$^{**}$  & 43.0$^{**}$ &	9.9 &	-3.0 &	8.9
 \\
BLEU & 1 & 25.6$^{*}$ &	23.5$^{*}$ &	29.9$^{**}$ &	17.6 &	6.3 &	5.9
\\
BERTScore-f & 1 & 48.5$^{**}$ &	46.8$^{**}$ &	61.4$^{**}$ &	18.5 &	5.0 &	17.1
 \\
\midrule
SARI & 10 & 34.4$^{**}$ &	29.9$^{**}$ &	51.9$^{**}$ &	26.3 &	11.4 &	53.2
  \\
SARI & 1 & 30.1$^{**}$ &	25.2$^{*}$ &	33.4$^{**}$ &	10.2 &	-2.7 &	8.4
\\
FKGL & 0 & 1.7 & 8.0  &	-12.0 &	16.2 &	-8.6 &	35.7
\\
BARTScore & 0 & 57.5 &	52.0 &	70.6 &	19.8 &	-14.3 &	32.6
  \\
PRISM & 0 & 56.8 &	45.1 &	71.0 &	8.1 &	-26.9 &	40.7
\\
QuestEval & 0 & 33.9 &	32.7 &	63.4 &	-4.1 &	-11.4 &	22.7\\

\midrule
\modelnamenoxs$_{\text{Simpl}\; W=\text{uniform}}$ & 0 & 50.5 & 43.6 & 67.5 & 1.3 & -35.8 & 24.1 \\
\modelnamenoxs$_{\text{Summ}\; W=\text{uniform}}$  & 0 & 48.6 &
40.3 & 66.7 & -8.0 & -39.8 & 21.0
\\
$\ \ \ \qquad\qquad\qquad_{W=\text{opt\_\texttt{Con}}}$  & 0 & 48.1 &
41.0 & 61.3 & -4.1 & -28.1 & 15.9 
\\
\ \ \ \qquad\qquad\qquad$_{W=\text{opt\_\texttt{Coh}}}$ & 0 & 35.4 & 26.2 & 57.0 & -9.6 & -34.6 & 31.3 
 \\
$\ \ \ \qquad\qquad\qquad_{W=\text{opt\_\texttt{Flu}}}$  & 0 & 55.7 & 48.6 & 57.0 & 21.1 & -4.3 & 16.3 \\
$\ \ \ \qquad\qquad\qquad_{W=\text{opt\_\texttt{Rel}}}$ & 0 &  46.6 & 37.3 & 66.5 & -12.4 & -39.4 & 22.5  \\
\bottomrule
\end{tabular}
\begin{tabular}{lccccccc}
\toprule
\multicolumn{8}{c}{\bf{Simplification subset (attention weight module's test set)}} \\
\midrule
{} & \bf{\#Ref} & \multicolumn{3}{c}{\bf{System-generated simplifications}} & \multicolumn{3}{c}{\bf{Human-written simplifications}}\\
& {} & Fluency & Simplicity & Meaning & Fluency & Simplicity & Meaning \\
\midrule
\modelnamenoxs$_{\text{Simpl}\; W=\text{uniform}}$ & 0 &  49.5 & 46.3 & 68.8 &  1.3 & -35.8 & 24.1
  \\
\modelnamenoxs$_{\text{Simpl}\; W=\text{learned}}$ & 0 & 33.9 & 28.5 & 54.0 & 7.0 & -30.5 & 30.8  \\
\bottomrule
\end{tabular}
    \caption{TODO: update caption} 
    \label{tab:simplification}
\end{table*}
